Attention-based Domain Adaptation for Single Stage Detectors

While domain adaptation has been used to improve the performance of object detectors when the training and test data follow different distributions, previous work has mostly focused on two-stage detectors. This is because their use of region proposals makes it possible to perform local adaptation, which has been shown to significantly improve the adaptation effectiveness. Here, by contrast, we target single-stage architectures, which are better suited to resource-constrained detection than two-stage ones but do not provide region proposals. To nonetheless benefit from the strength of local adaptation, we introduce an attention mechanism that lets us identify the important regions on which adaptation should focus. Our method gradually adapts the features from global, image-level to local, instance-level. Our approach is generic and can be integrated into any single-stage detector. We demonstrate this on standard benchmark datasets by applying it to both SSD and YOLOv5. Furthermore, for equivalent single-stage architectures, our method outperforms the state-of-the-art domain adaptation techniques even though they were designed for specific detectors.

==> figures/attention_mod.tex <==
% !TEX root = ../top_sup.tex
% !TEX spellcheck = en-US
\begin{figure}[t]
\centering
\begin{tabular}{c}
\includegraphics[width=.45\linewidth]{figures/attn_module.png}
\end{tabular}
  \caption{{\bf Self Attention Module}: Following~\cite{detr}, we use multihead attention followed by a feed forward network.} 

  \label{fig:attn_mod}
  \end{figure}

==> figures/domain_samples_city_foggy.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
\centering
\begin{tabular}{c}
\includegraphics[width=\linewidth]{figures/city_foggy}
% \includegraphics[width=.45\linewidth]{figures/city_foggy}\\
\end{tabular}
\vspace{-1cm}
  \caption{{\bf Sample images from Cityscapes (top) and Foggy Cityscapes (bottom).} This illustrates a challenging domain shift, where weather conditions, and thus appearance, differ significantly between both domains.}
 
  \label{fig:sample_domain_city_foggy}
  \end{figure}


==> figures/domain_samples_sim_kitti.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
\centering
\begin{tabular}{c}
\includegraphics[width=\linewidth]{figures/sim_kitti}
% \includegraphics[width=.45\linewidth]{figures/city_foggy}\\


\end{tabular}
  \caption{{\bf Sample images from Sim10k (top) and KITTI (bottom).} These images highlight the appearance discrepancies between synthetic and real data.}
 
  \label{fig:sample_domain_sim_kitti}
  \end{figure}
  

==> tables/city2foggy.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table*}[t]
	\centering 
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
	\hline
	Method & person & car  & train  & rider  & truck  & motorcycle & bicycle & bus & mAP@0.5\\
	\hline 
	\hline 
	~\cite{hsu2020every} - no DA &  &   &   &   &   &  &  &  &13.9   \\ 
	\hline
	~\cite{hsu2020every} &  &   &   &   &   &  &  &  &23.5\\
	\hline
	SSD - no DA &  &   &   &   &   &  &  &  &13.2\\
	\hline
	SSD + our DA &  &   &   &   &   &  &  &  &\textbf{23.9}\\ 
	\hline
	YOLO - no DA &  &   &   &   &   &  &  &  & 10.6\\
	\hline
	YOLO + our DA &  &   &   &   &   &  &  &  & 17.2\\
	\hline
	\end{tabular}
	\caption{Results on Cityscapes to Foggy adaptation}
	\label{tab:city2foggy}
\end{table*}

==> tables/city2foggy_yolo.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table*}[t]
	\centering 
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
	\hline
	\hline
	Method & person & car  & train  & rider  & truck  & motorcycle & bicycle & bus & mAP@0.5\\
	\hline 
	\hline
	YOLO - w/o DA & \textbf{19.8}  &27.2   & 1.5  & \textbf{22.5}  & 1.5  & \textbf{2.5} & \textbf{15.8} & 1.8 & \textbf{11.6}\\
	\hline
	YOLO w/o attn w DA &17.2 &29.6   & 0  &15.7   & \textbf{4.3}  & 0 &12.7  &\textbf{8.2}  & 11.1\\
	\hline
	YOLO + our DA & 16.2 &\textbf{30.3}   &0   &20  &1.3   & 1.2 &13.5  & 7.2  & 11.2\\
	\hline
	\end{tabular}
	\caption{Results on Cityscapes to Foggy adaptation}
	\label{tab:city2foggyyolo}
\end{table*}

==> tables/kitti2city.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
	\centering 
	\begin{tabular}{|c|c|}
	\hline
	Method & mAP@0.5\\
	\hline 
	\hline 
	~\cite{hsu2020every} - w/0 DA & 33.3\\ 
	\hline
	~\cite{hsu2020every} & 27.8\\
	\hline
	SSD - no DA & 33.1\\
	\hline
	SSD + our DA & \textbf{40.2}\\ 
	\hline
	YOLO - no DA & 22.5 \\
	\hline
	YOLO + our DA & 32.8\\
	\hline
	\end{tabular}
	\caption{Results on KITTI to Cityscapes adaptation}
	\label{tab:kitti2city}
\end{table}

==> tables/kitti2city_yolo.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
	\centering 
	\begin{tabular}{|c|c|}
	\hline
	Method & mAP@0.5\\
	\hline
	YOLO - w/o DA & 13.7 \\
	\hline
	YOLO - w/o attn w DA & 29.6 \\
	\hline
	YOLO + our DA & \textbf{31.1}\\
	\hline
	\end{tabular}
	\caption{Results on KITTI to Cityscapes adaptation}
	\label{tab:kitti2city_yolo}
\end{table}

==> tables/sim2city.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
	\centering 
	\begin{tabular}{|c|c|}
	\hline
	Method & mAP@0.5\\
	\hline 
	\hline 
	~\cite{hsu2020every} - no DA & 31.5\\ 
	\hline
	~\cite{hsu2020every} & 32.8\\
	\hline
	SSD - no DA & 29.1\\
	\hline
	SSD + our DA & \textbf{34.8}\\ 
	\hline
	YOLO - no DA & 32 \\
	\hline
	YOLO + our DA & 33.2\\
	\hline
	\end{tabular}
	\caption{Results on Sim10K to Cityscapes adaptation}
	\label{tab:sim2city}
\end{table}

==> tables/sim2city_yolo.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
	\centering 
	\begin{tabular}{|c|c|}
	\hline
	Method & mAP@0.5\\
	\hline
	YOLO - w/o DA & 29.2 \\
	\hline
	YOLO - w/o attn w DA & 33.4\\
	\hline
	YOLO + our DA & \textbf{34.4}\\
	\hline
	\end{tabular}
	\caption{Results on Sim10K to Cityscapes adaptation}
	\label{tab:sim2cityyolo}
\end{table}
